LTL2Action: Generalizing LTL Instructions for Multi-Task RL

We address the problem of teaching a deep reinforcement learning (RL) agent to follow instructions in multi-task environments. Instructions are expressed in a well-known formal language -- linear temporal logic (LTL) -- and can specify a diversity of complex, temporally extended behaviours, including conditionals and alternative realizations. Our proposed learning approach exploits the compositional syntax and the semantics of LTL, enabling our RL agent to learn task-conditioned policies that generalize to new instructions, not observed during training. To reduce the overhead of learning LTL semantics, we introduce an environment-agnostic LTL pretraining scheme which improves sample-efficiency in downstream environments. Experiments on discrete and continuous domains target combinatorial task sets of up to $\sim10^{39}$ unique tasks and demonstrate the strength of our approach in learning to solve (unseen) tasks, given LTL instructions.

==> figures/generalization-new.tex <==
\begin{table*}[t]
\small
\centering
\caption{
% \commental{I don't think we should label the training distribution with I.I.D. All the samplers are technically I.I.D. from some distribution. Maybe "Same Distr." or what we originally had? } \commentpv{Not sure why \grupp is missing here?} 
Trained RL agents are evaluated on increased depth (depth: 15, conjuncts: 2-4) and increased number of conjuncts (depth: 3-5, conjuncts: 12) partially-ordered tasks. 
In each entry, we report \textit{total reward} and 100 $\times$ \textit{discounted return} (in parentheses) with 90\% confidence error, averaged over 30 seeds and 100 episodes per seed.}
\label{table:generalization-new}

\begin{tabular}{*{3}c}
% \addlinespace[-\aboverulesep] 
\cmidrule[\heavyrulewidth]{2-3} 
& \multicolumn{1}{c}{$\uparrow$ Depth ($3\times)$} &
  \multicolumn{1}{c}{$\uparrow$ Conjuncts ($3\times)$} \\ 
%   \cmidrule[\heavyrulewidth]{2-3}
% & \multicolumn{3}{c}{(a) Avoidance Tasks} \\ \cmidrule(lr){2-4} 
% \multicolumn{1}{l}{\gnnpp} &  0.97(0.65) & \textbf{0.99}(\textbf{0.35}) & 0.64(0.18)  \\ 
% \multicolumn{1}{l}{\gnnp} & \textbf{0.98}(\textbf{0.66}) & 0.98(0.33)   & 0.57(0.14) \\ 
% % \multicolumn{1}{l}{\grupp} &   0.95(0.62)  &  0.56(0.12)   & 0.55(0.13)  \\ 
% \multicolumn{1}{l}{\grup} & 0.97(0.65)          & 0.40(0.06)   & \textbf{0.67}(\textbf{0.22})  \\ 
% \multicolumn{1}{l}{GRU}             & 0.32(0.22)          & -0.03(-0.01) & -0.35(-0.16) \\ 
% \multicolumn{1}{l}{Myopic}          & 0.82(0.42)          & 0.41(0.01)   & 0.32(-0.05)\\% \bottomrule

% \addlinespace[-\aboverulesep] 
 \cmidrule{2-3} &
  \multicolumn{2}{c}{(b) Partially-Ordered Tasks} \\ 
%   \cmidrule(lr){2-4} &
%   \multicolumn{1}{c}{I.I.D} &
%   \multicolumn{1}{c}{$\uparrow$ Depth} &
%   \multicolumn{1}{c}{$\uparrow$ Conjuncts} \\ 
  \cmidrule{2-3}
\multicolumn{1}{l}{\gnnpp} &  $\mathbf{0.979} \pm 0.004$ $(\mathbf{0.876} \pm 0.0003)$ & $0.992 \pm 0.003$ $( \mathbf{3.800} \pm 0.081)$ \\ 
\multicolumn{1}{l}{\gnnp}  & $0.974 \pm 0.005$ $(0.742 \pm 0.027)$  & $0.983 \pm 0.004$ $(3.399 \pm 0.081)$ \\ 
\multicolumn{1}{l}{\grup}  &  $0.249 \pm 0.013$ $(0.044 \pm 0.006)$ & $0.991 \pm 0.003$  $(2.211 \pm 0.067)$\\ 
\multicolumn{1}{l}{GRU}    & $0.030 \pm 0.005$  $(0.001 \pm 0.000)$ & $0.538 \pm 0.015$ $(0.749 \pm 0.045)$ \\ 
\multicolumn{1}{l}{Myopic} & $0.959 \pm 0.006$ $(0.445 \pm 0.018)$ & $\mathbf{0.999} \pm 0.001$ $(2.425 \pm 0.057)$  \\ \bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}


% \begin{table*}[t]
% \small
% \centering
% \caption{
% % \commental{I don't think we should label the training distribution with I.I.D. All the samplers are technically I.I.D. from some distribution. Maybe "Same Distr." or what we originally had? } \commentpv{Not sure why \grupp is missing here?} 
% Trained RL agents are evaluated on the training distribution of tasks, as well as out-of-distribution tasks with increased depth of sequences, and increased number of conjuncts. In each entry, we report \textit{total reward} and \textit{discounted return} (in parentheses) averaged over 30 seeds and 100 episodes per seed.}
% \label{table:generalization}

% \begin{tabular}{*{4}c}
% % \addlinespace[-\aboverulesep] 
% % \cmidrule[\heavyrulewidth]{2-4} 
% & \multicolumn{1}{c}{I.I.D} &
%   \multicolumn{1}{c}{$\uparrow$ Depth ($3\times)$} &
%   \multicolumn{1}{c}{$\uparrow$ Conjuncts ($3\times)$} \\ \cmidrule[\heavyrulewidth]{2-4}
% % & \multicolumn{3}{c}{(a) Avoidance Tasks} \\ \cmidrule(lr){2-4} 
% % \multicolumn{1}{l}{\gnnpp} &  0.97(0.65) & \textbf{0.99}(\textbf{0.35}) & 0.64(0.18)  \\ 
% % \multicolumn{1}{l}{\gnnp} & \textbf{0.98}(\textbf{0.66}) & 0.98(0.33)   & 0.57(0.14) \\ 
% % % \multicolumn{1}{l}{\grupp} &   0.95(0.62)  &  0.56(0.12)   & 0.55(0.13)  \\ 
% % \multicolumn{1}{l}{\grup} & 0.97(0.65)          & 0.40(0.06)   & \textbf{0.67}(\textbf{0.22})  \\ 
% % \multicolumn{1}{l}{GRU}             & 0.32(0.22)          & -0.03(-0.01) & -0.35(-0.16) \\ 
% % \multicolumn{1}{l}{Myopic}          & 0.82(0.42)          & 0.41(0.01)   & 0.32(-0.05)\\% \bottomrule

% % \addlinespace[-\aboverulesep] 
%  \cmidrule{2-4} &
%   \multicolumn{3}{c}{(b) Partially-Ordered Tasks} \\ 
% %   \cmidrule(lr){2-4} &
% %   \multicolumn{1}{c}{I.I.D} &
% %   \multicolumn{1}{c}{$\uparrow$ Depth} &
% %   \multicolumn{1}{c}{$\uparrow$ Conjuncts} \\ 
%   \cmidrule{2-4}
% \multicolumn{1}{l}{\gnnpp} &   & $\mathbf{0.991} \pm 0.003$ $(\mathbf{0.033} \pm 0.001)$ & $\mathbf{0.999} \pm 0.001$ $(\mathbf{0.083} \pm 0.002)$ \\ 
% \multicolumn{1}{l}{\gnnp}  &   & $0.985 \pm 0.004$ $(0.031 \pm 0.001)$  & $0.997 \pm 0.002$ $(0.078 \pm 0.002)$ \\ 
% \multicolumn{1}{l}{\grup}  &   & $0.442 \pm 0.015$ $(0.012 \pm 0.001)$ & $0.998 \pm 0.001$  $(0.060 \pm 0.002)$\\ 
% \multicolumn{1}{l}{GRU}    &  & $0.072 \pm 0.008$ $(0.000 \pm 0.000)$ & $0.706 \pm 0.014$ $(0.021 \pm 0.001)$ \\ 
% \multicolumn{1}{l}{Myopic} &  & $0.971\pm 0.001$ $(0.021 \pm 0.001)$ & $\mathbf{0.999}\pm0.000$ $(0.052 \pm 0.001)$  \\ \bottomrule
% \end{tabular}
% \vspace{-5mm}
% \end{table*}


% % {
% % \centering
% % \begin{table*}[h]
% % \begin{tabular}{@{}l|l|l|l|l|l|l|@{}}
% % \cmidrule(l){2-7}
% %                                       & \multicolumn{3}{c|}{Avoidance Tasks}                        & \multicolumn{3}{c|}{Partially-Ordered Tasks}       \\ \cmidrule(l){2-7} 
% %  &
% %   \multicolumn{1}{c|}{Train distr.} &
% %   \multicolumn{1}{c|}{$\uparrow$ Depth} &
% %   \multicolumn{1}{c|}{$\uparrow$ Conjuncts} &
% %   \multicolumn{1}{c|}{Train distr.} &
% %   \multicolumn{1}{c|}{$\uparrow$ Depth} &
% %   \multicolumn{1}{c|}{$\uparrow$ Conjuncts} \\ \midrule
% % \multicolumn{1}{|l|}{GNN+progression+pretraining} &
% %   0.97 , 0.65 &
% %   \textbf{0.99} , \textbf{0.35} &
% %   0.64 , 0.18 &
% %   \textbf{1.0} , \textbf{0.48} &
% %   \textbf{0.998} , \textbf{0.20} &
% %   \textbf{1.0} , \textbf{0.23} \\ \midrule
% % \multicolumn{1}{|l|}{GNN+progression} & \textbf{0.98} , \textbf{0.66} & 0.98 , 0.33   & 0.57 , 0.14          & \textbf{1.0} , 0.47  & 0.996 , 0.19 & 0.999 , 0.22 \\ \midrule
% % \multicolumn{1}{|l|}{GRU+progression} & 0.97 , 0.65          & 0.40 , 0.06   & \textbf{0.67} , \textbf{0.22} & \textbf{1.0} , 0.46  & 0.90 , 0.16  & 0.995 , 0.21 \\ \midrule
% % \multicolumn{1}{|l|}{GRU}             & 0.32 , 0.22          & -0.03 , -0.01 & -0.35 , -0.16        & 0.87 , 0.24 & 0.24 , 0.02  & 0.66 , 0.07  \\ \midrule
% % \multicolumn{1}{|l|}{Myopic}          & 0.82 , 0.42          & 0.41 , 0.01   & 0.32 , -0.05         & \textbf{1.0} , 0.40  & 0.98 , 0.14  & 0.999 , 0.16 \\ \bottomrule
% % \end{tabular}
% % \caption{Trained RL agents are evaluated on the training distribution of tasks, as well as out-of-distribution tasks with increased depth of sequences, and increased number of conjuncts. In each entry, we report (\textit{Total Reward} , \textit{Discounted Return}) averaged over 30 seeds and 100 episodes per seed. The highest values in each set of tasks is in bold.}
% % \label{table:generalization}
% % \end{table*}
% % }


% % % Please add the following required packages to your document preamble:
% % % \usepackage{booktabs}
% % % \usepackage{multirow}
% % \begin{table}[]
% % \begin{tabular}{@{}l|l|l|l|l|l|l|l@{}}
% % \cmidrule(l){2-8}
% %  &
% %   \multicolumn{1}{c|}{\multirow{2}{*}{Metric}} &
% %   \multicolumn{3}{c|}{Avoidance Tasks} &
% %   \multicolumn{3}{c|}{Parallel Tasks} \\ \cmidrule(l){3-8} 
% %  &
% %   \multicolumn{1}{c|}{} &
% %   \multicolumn{1}{c|}{Training distr.} &
% %   \multicolumn{1}{c|}{Longer} &
% %   \multicolumn{1}{c|}{More conjunctions} &
% %   \multicolumn{1}{c|}{Training distr.} &
% %   \multicolumn{1}{c|}{Longer} &
% %   \multicolumn{1}{c|}{More conjunctions} \\ \midrule
% % \multicolumn{1}{|l|}{\multirow{2}{*}{GNN+progression+pretraining}} &
% %   Total return &
% %   0.972 (0.007) &
% %   \textbf{0.99 (0.004)} &
% %   0.636 (0.023) &
% %   \textbf{1.0 (0)} &
% %   \textbf{0.998 (0.001)} &
% %   \multicolumn{1}{l|}{\textbf{1.0 (0)}} \\
% % \multicolumn{1}{|l|}{} &
% %   Discounted return &
% %   0.652 (0.007) &
% %   \textbf{0.345 (0.003)} &
% %   0.176 (0.014) &
% %   \textbf{0.475 (0.006)} &
% %   \textbf{0.195 (0.004)} &
% %   \multicolumn{1}{l|}{\textbf{0.229 (0.003)}} \\ \midrule
% % \multicolumn{1}{|l|}{\multirow{2}{*}{GNN+progression}} &
% %   Total return &
% %   \textbf{0.983 (0.006)} &
% %   0.981 (0.004) &
% %   0.573 (0.025) &
% %   \textbf{1.0 (0)} &
% %   0.996 (0.002) &
% %   \multicolumn{1}{l|}{0.999 (0.001)} \\
% % \multicolumn{1}{|l|}{} &
% %   Discounted return &
% %   \textbf{0.658 (0.006)} &
% %   0.328 (0.004) &
% %   0.143 (0.015) &
% %   0.470 (0.006) &
% %   0.192 (0.004) &
% %   \multicolumn{1}{l|}{0.222 (0.003)} \\ \midrule
% % \multicolumn{1}{|l|}{\multirow{2}{*}{GRU+progression}} &
% %   Total return &
% %   0.973 (0.007) &
% %   0.403 (0.016) &
% %   \textbf{0.667 (0.022)} &
% %   \textbf{1.0 (0)} &
% %   0.901 (0.009) &
% %   \multicolumn{1}{l|}{0.995 (0.002)} \\
% % \multicolumn{1}{|l|}{} &
% %   Discounted return &
% %   0.646 (0.007) &
% %   0.059 (0.005) &
% %   \textbf{0.216 (0.013)} &
% %   0.459 (0.006) &
% %   0.158 (0.005) &
% %   \multicolumn{1}{l|}{0.205 (0.004)} \\ \midrule
% % \multicolumn{1}{|l|}{\multirow{2}{*}{GRU}} &
% %   Total return &
% %   0.320 (0.019) &
% %   -0.026 (0.006) &
% %   -0.348 (0.015) &
% %   0.873 (0.010) &
% %   0.235 (0.013) &
% %   \multicolumn{1}{l|}{0.661 (0.014)} \\
% % \multicolumn{1}{|l|}{} &
% %   Discounted return &
% %   0.215 (0.012) &
% %   -0.008 (0.002) &
% %   -0.157 (0.009) &
% %   0.238 (0.007) &
% %   0.015 (0.001) &
% %   \multicolumn{1}{l|}{0.068 (0.003)} \\ \midrule
% % \multicolumn{1}{|l|}{\multirow{2}{*}{Myopic}} &
% %   Total return &
% %   0.824 (0.016) &
% %   0.409 (0.020) &
% %   0.321 (0.027) &
% %   \textbf{1.0 (0)} &
% %   0.980 (0.004) &
% %   \multicolumn{1}{l|}{0.999 (0.001)} \\
% % \multicolumn{1}{|l|}{} &
% %   Discounted return &
% %   0.424 (0.012) &
% %   0.014 (0.004) &
% %   -0.046 (0.011) &
% %   0.401 (0.007) &
% %   0.140 (0.004) &
% %   \multicolumn{1}{l|}{0.157 (0.003)} \\ \bottomrule
% % \end{tabular}
% % \end{table}

==> sections/01-intro.tex <==
\section{Introduction}

% Instructing AI agents, a long-standing dream for AI
% RL and deep learning presents a path to do so (policies that are conditioned on natural language instructions). In principle, this approach could lead to policies that generalize to unseen instructions in a zero-shot learning fashion. Unfortunately, this approach does not scale well.
A long-standing aspiration of artificial intelligence is to build agents that can understand and follow human instructions to solve problems \cite{mccarthy1960programs}.
Recent advances in deep learning \cite{goodfellow2016deep} and reinforcement learning (RL) \cite{sutton2018reinforcement} provide a vehicle to achieve this ambition. Using deep RL, it is possible to learn a policy that decides the next action conditioned on the current observation and a natural language instruction. Given enough training data, the learned policy will show some degree of generalization to unseen instructions (without further training), as shown by previous works \citep[e.g.,][]{DBLP:journals/corr/HermannHGWFSSCJ17,DBLP:conf/icml/OhSLK17,DBLP:conf/aaai/ChaplotSPRS18,DBLP:conf/iclr/YuZX18,DBLP:conf/iclr/Co-ReyesGSAADAL19,DBLP:conf/nips/JiangGMF19,DBLP:conf/ijcai/LuketinaNFFAGWR19}. Unfortunately, this approach does not scale well because it requires (for every possible environment) manually building a large training set comprised of natural language instructions with their corresponding reward functions.



% Alternative is to use a more structured (but still flexible) language, that allows for automatically generating reward functions for each instruction. E.g., sketches, task graphs, programs, LTL. In other words, using these languages we can automatically generate infinite data to train our policy. Some of these languages are more expressive or more intuitive than others. Approaches that use those languages rely on hierarchical RL to decompose problems. For that reason, they converge to suboptimal solutions (myopic solutions).
Motivated by this observation, recent works have explored using formal languages (instead of natural language) to instruct RL agents. 
% PREVIOUS %The main advantage of using a formal language is that its semantics are unambiguous and, hence, its corresponding reward functions can be automatically generated. 
Formal languages offer several desirable properties for RL, including unambiguous semantics, compact syntax, and automatic reward function generation.
This allows RL practitioners to generate infinite training data (automatically) to teach RL agents to follow instructions. Some examples of such formal languages are policy sketches \cite{andreas2017modular}, task graphs \cite{DBLP:conf/nips/SohnOL18}, procedural programs \cite{DBLP:conf/iclr/SunWL20}, declarative programs \cite{DBLP:journals/corr/DenilCCSF17}, reward machines \cite{DBLP:journals/corr/abs-2010-03950}, and temporal logic  \cite{leon2020systematic}. A common theme within this body of literature is to decompose the overall instruction into smaller subtasks that are solved independently. For instance, if one task is ``\textit{do task-A and then task-B}" and another task is ``\textit{do task-A and then task-C}," these approaches will reuse the same policy to achieve \textit{task-A}. Unfortunately, doing so might lead to suboptimal behaviour because the optimal way to achieve \textit{task-A} depends on what the agent has to do next (e.g., if \textit{task-A} consists of getting coffee and there are multiple coffee machines, then the optimal coffee machine to use depends on where the agent has to go after getting the coffee). We call these approaches \emph{myopic} as they %\remove{myopically} 
optimize the completion of subtasks without considering the rest of the task.

%\commentsm{LTL progression is not a "property" of LTL. In our context, progression is a rewriting operation, that preserves certain properties of the LTL formula and (I believe) is made possible by the fact that LTL is a formal language with a compositional syntax. Also beware that "progression" and "regression" are used with dynamical systems to talk in another way. I can take a stab at rephrasing. }
% What we did
% V1
%In this work, we use \emph{linear temporal logic (LTL)} \cite{DBLP:conf/focs/Pnueli77} to instruct RL agents and exploit a fundamental property of LTL, called \emph{LTL progression}, to learn policies that generalize well to unseen instructions without compromising convergence guarantees -- in contrast to myopic approaches. LTL is an expressive formal language that allows for specifying tasks as goal sequences, partial-order tasks, and safety constraints, among others. \remove{LTL has many nice properties and we exploit one particularly powerful property in this work, known as LTL progression.} LTL progression allows the agent to consume an LTL instruction as it makes progress towards solving the task. For instance, if the task is ``\textit{do task-A and then task-B}," then the formula can be automatically progressed to ``\textit{do task-B}" as soon as the agent completes \textit{task-A}. This allows the agent to reduce the complexity of the task being solved over time, which supports generalization.
% V2
In this work, we use \emph{linear temporal logic (LTL)} \cite{DBLP:conf/focs/Pnueli77} to instruct RL agents and exploit a rewriting operation, called \emph{LTL progression}, to learn policies that generalize well to unseen instructions without compromising convergence guarantees -- in contrast to myopic approaches. LTL is an expressive formal language that allows for specifying tasks as goal sequences, partial-order tasks, and safety constraints, among others. LTL progression allows the agent to consume an LTL instruction as it makes progress towards solving the task. For instance, if the task is ``\textit{do task-A or task-B, and then task-C}," then the formula can be automatically progressed to ``\textit{do task-C}" as soon as the agent completes \textit{task-A} or \textit{task-B}. This allows the agent to reduce the complexity of the task being solved over time, which supports generalization.
%\commentsm{"do task-A or task-B and then task-C" is almost as simple but shows the value of LTL (or other expressive formal languages) over sequences.}

% The contribution of our work are the following:
% V1
%In more details, our approach requires a predefined set of \textit{event detectors}. These detectors indicate when different subtasks are completed in the environment. Then, we use LTL to compose occurrences of those detectors over time to define complex tasks. Given the detectors, we can randomly sample millions of LTL tasks for the agent to learn from. We then show how to transforms LTL tasks into their corresponding reward functions by rewarding the agent when the task is completed. Finally, we use deep RL to learn a policy that considers the current observation and LTL instructions when selecting actions. Crucially, we progress the LTL instruction as the agent interacts with the environment. Results on discrete and continuous domains show that progressing the LTL task leads to better generalization performance than following a myopic approach. In addition, we show that the LTL tasks can be encoded using an LSTM, GRU, or a graph neural network (GNN), and that all those encoders work well in practice. That said, our best results were obtained by encoding the LTL task using a GNN. Finally, we show that the LTL encoder can be pretrained in an environment-agnostic fashion and that doing so results on an extra boost in generalization performance \commental{Pretraining doesn't seem to impact upward generalization, only the sample efficiency (which can be considered generalization from a small amount of data). We should consider making this clear though}. With that, the main contributions of our paper can be summarized as follows:
% V2
In more details, our approach requires a predefined set of \textit{event detectors}. These detectors indicate when different subtasks are completed in the environment. Then, we use LTL to compose occurrences of those detectors over time to define complex tasks. Given the detectors, we can randomly sample millions of LTL tasks for the agent to learn from. We then show how to transforms LTL tasks into their corresponding reward functions by rewarding the agent when the task is completed. Finally, we use deep RL to learn a policy that considers the current observation and LTL instructions when selecting actions. Crucially, we progress the LTL instruction as the agent interacts with the environment. Results on discrete and continuous domains show that progressing the LTL task leads to better generalization performance than following a myopic approach. In addition, we show that the LTL tasks can be encoded using an LSTM, GRU, or a graph neural network (GNN), and that all those encoders work well in practice. That said, our best results were obtained by encoding the LTL task using a GNN. Finally, we show that the LTL encoder can be pretrained in an environment-agnostic fashion and that doing so results on better sample efficiency.  %\commental{Pretraining doesn't seem to impact upward generalization, only the sample efficiency (which can be considered generalization from a small amount of data). We should consider making this clear though}.
With that, the main contributions of our paper can be summarized as follows:
\begin{itemize}
    \setlength\itemsep{0em}
    %\item A novel approach for teaching RL agents to \remove{understand} LTL instructions and generalize to unseen instructions without requiring further training. Our approach has theoretical advantages over existing methods to instruct RL agents using LTL  \cite{kuo2020encoding,leon2020systematic}. This derives on a better generalization performance in our experiments. 
    \item A novel approach for teaching RL agents to follow LTL instructions. Our approach has theoretical advantages over existing methods to instruct RL agents using LTL  \cite{kuo2020encoding,leon2020systematic}. This derives on a better generalization performance in our experiments. 
    \item Empirical results comparing different methods to encode LTL instructions (LSTM, GRU, GNN).
    \item To show that the LTL encoder can be pretrained in an environment-agnostic manner and the empirical advantages of doing so.
\end{itemize}



% \commental{What are the theoretical advantages of our approach over Kuo et al?} 
%     \commentrti{While we solve a Markovian problem, they solve a partially observable problem. As Littman said once to me, ``MDPs are easy, POMDPs are hard." Not sure if our current discussion about Kuo et al makes this distinction clear in the body of the paper, though.} \commental{Makes sense, thanks. :)}
    
%While any RL method can be used for learning such a policy, we use PPO because it has been shown to generalize well to unseen situations \textbf{[citation needed]}. To encode the LTL instructions, we use an 



%   - We propose a novel approach for zero-shot generalization based on LTL progression
%   - Converge guarantees(?)
%   - LSTM, GRU, and GNN encoders (show that it works well using these different encoders?)
%   - Results on discrete and continuous domains
% (*) Maybe say that we are using PPO and why (?)

% RL is cool but:
%    - they only understand rewards
%    - they learn a policy that can solve one task
% Instructing RL agents
% ... we explore how to instruct RL agents (and how to achieve zero-shot generalization)

% Previous work using natural language and multigoal RL
% Problem: 
%   - generation of large training set
%   - performance? progression?

% natural language \cite{DBLP:conf/nips/JiangGMF19}
%   - They actually just use language to describe goal states (instead of using a goal state)
%   - To solve more complex tasks, they use HRL -- but the HRL approach does not generalize or receives instructions. It just uses the low-level policies by feeding them "natural language instructions" instead of goal states (but technically they just predefined a set of possible "goal instructions" for the HRL module to pick from)
%   - Requires to manually construct a large training set of "textual descriptions" and corresponding "reward functions".

% Programs \cite{DBLP:conf/iclr/SunWL20}:
%   - Myopic
%   - Requires separate definitions for perception primitives (i.e., event detectors) and action primitives (i.e., subtasks).
%   - They trained the perception primitives using supervised learning.
%   - They must define a reward function for each program. This is expensive (in fact, they only have 4000 training programs while we can automatically generate an infinite training set).
%   - Tasks kind of progress since the program works as the memory.

% Here we propose to instruct agents using LTL. Advantages:
%   - Expressive power
%   - Automatic mapping from LTL to rewards (which allows to automatically create huge training sets)
%   - LTL progression allows automatic "check"

% Previous work had explore using LTL to define reward function, but our focus here is in generalization
% Two recent works have explore how to train an RL agent to follow unseen LTL instructions, but they do not exploit LTL progression or they might converge to suboptimal policies. We empirically show that we are better than that :P

% Possible things to highlight:

% - Framing our work within the broader context of "combining deep RL with symbolic methods"

% - LTL can express complex temporally-extended behaviours, while most other frameworks only consider sequential tasks

% - The significance of learning policies which generalize to unseen tasks
